Using quantile time series and historical simulation to forecast financial risk multiple steps ahead

A method for quantile-based, semi-parametric historical simulation estimation of multiple step ahead Value-at-Risk (VaR) and Expected Shortfall (ES) models is developed. It uses the quantile loss function, analogous to how the quasi-likelihood is employed by standard historical simulation methods. The returns data are scaled by the estimated quantile series, then resampling is employed to estimate the forecast distribution one and multiple steps ahead, allowing tail risk forecasting. The proposed method is applicable to any data or model where the relationship between VaR and ES does not change over time and can be extended to allow a measurement equation incorporating realized measures, thus including Realized GARCH and Realized CAViaR type models. Its finite sample properties, and its comparison with existing historical simulation methods, are evaluated via a simulation study. A forecasting study assesses the relative accuracy of the 1% and 2.5% VaR and ES one-day-ahead and ten-day-ahead forecasting results for the proposed class of models compared to several competitors.

==> all-assets.10days.tex <==
\begin{table}[hbt]
\caption{\small 10-day risk forecasting results: average values across all assets. Key to table: \emph{Est.}: estimation method; \emph{Q$\alpha$}; average quantile loss value at the $\alpha\%$ ; \emph{J$\alpha$}; average joint loss value at the $\alpha\%$; \emph{R(L$\alpha$)}: average ranking of models under loss L at level $\alpha$; \emph{M(L$\alpha$)}: MCS p-value under loss L$\alpha$ (in brackets: number of times a model is included in the MCS); \emph{M(all)}: number of times a model is included in the MCS overall.\\}
\label{tab:allassets10day}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.65}
\small
%\begin{tabularx}{\textwidth}{*{15}{>{\centering\arraybackslash}X}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccc}
\hline
Est.          & Model   & Q2.5                           & J2.5                          & Q1                             & J1                            & R(Q2.5)                    & R(J2.5)                    & R(Q1)                      & R(J1)                      & M(Q2.5)                          & M(J2.5)                          & M(Q1)                            & M(J1)                            & M(all)                    \\ \hline
\textbf{ML}   & GHS     & \textbf{155.62}               & 3.874                        & 72.66                        & 4.002      & \textbf{25.7}              & \textbf{23.3}              & 17.7                       & 19.3                       & $\underset{(1)}{0.155}$          & $\underset{(0)}{0.071}$          & $\underset{(0)}{0.026}$          & $\underset{(1)}{0.221}$          & 2                         \\
              & GJ-HS   & 152.85                        & 3.825                        & 69.88                        & 3.931      & 22.7                       & 16.5                       & 10.7                       & 9.8                        & $\underset{(2)}{0.277}$          & $\underset{(1)}{0.263}$          & $\underset{(0)}{0.113}$          & $\underset{(1)}{0.323}$          & 4                         \\ \hline
\textbf{QL}   & IG1     & 154.10                        & 3.835                        & 70.31                        & 3.975      & 20.0                       & 17.3                       & 11.3                       & 15.7                       & $\underset{(1)}{0.297}$          & $\underset{(1)}{0.330}$          & $\underset{(0)}{0.019}$          & $\underset{(1)}{0.299}$          & 3                         \\
              & 2.5     & 150.96 &	3.820 &	71.35 &	3.966      & 16.3                       & 15.5                       & 15.0                       & 16.7                       & $\underset{(0)}{0.212}$          & $\underset{(0)}{0.103}$          & $\underset{(0)}{0.021}$          & $\underset{(1)}{0.256}$          & \textbf{1}                \\
              & 5       & 150.98 &	3.824 &	72.79 &	3.983      & 18.3                       & 17.0                       & 18.3                       & 19.3                       & $\underset{(2)}{0.242}$          & $\underset{(1)}{0.139}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.254}$          & 4                         \\
              & 10      & 153.65 &	3.840 &	73.26 &	3.990                         & 23.7                       & 20.7                       & 19.0                       & 17.8                       & $\underset{(1)}{0.159}$          & $\underset{(0)}{0.071}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(0)}{0.097}$          & \textbf{1}                \\
              & 15      & 152.58 &	3.828 &	72.68 &	3.974                        & 20.0                       & 18.3                       & 16.0                       & 14.3                       & $\underset{(0)}{0.169}$          & $\underset{(0)}{0.107}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.189}$          & \textbf{1}                \\
              & 20      & 152.93 &	3.827 &	72.68 &	3.972                       & 21.3                       & 18.0                       & 17.0                       & 14.2                       & $\underset{(0)}{0.171}$          & $\underset{(0)}{0.117}$          & $\underset{(0)}{0.055}$          & $\underset{(1)}{0.155}$          & \textbf{1}                \\
              & IGJR1   & 154.48 &	3.834 &	71.92 &	3.963                        & 20.7                       & 17.8                       & 16.3                       & 15.0                       & $\underset{(0)}{\textbf{0.137}}$ & $\underset{(1)}{0.161}$          & $\underset{(0)}{0.045}$          & $\underset{(1)}{0.303}$          & 2                         \\
              & 2.5     & 151.80 &	3.825 &	72.98 &	3.989                        & 17.7                       & 15.5                       & 19.0                       & 19.7                       & $\underset{(1)}{0.285}$          & $\underset{(1)}{0.306}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.260}$          & 3                         \\
              & 5       & 152.34 &	3.830 &	73.59 &	3.993                       & 22.0                       & 18.3                       & 19.3                       & 19.2                       & $\underset{(1)}{0.145}$          & $\underset{(0)}{\textbf{0.061}}$ & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(0)}{0.059}$          & \textbf{1}                \\
              & 10      & 151.06 &	3.822 &	74.44 &	3.997                     & 18.0                       & 16.3                       & \textbf{21.3}              & 20.2                       & $\underset{(1)}{0.161}$          & $\underset{(0)}{0.076}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(0)}{\textbf{0.051}}$ & \textbf{1}                \\
              & 15      & 150.98 &	3.824 &	74.29 &	4.005                      & 16.3                       & 16.0                       & 20.3                       & 20.0                       & $\underset{(1)}{0.185}$          & $\underset{(0)}{0.110}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.115}$          & 2                         \\
              & 20      & 150.37 &	3.812 &	73.99 &	3.985                        & 15.3                       & 14.2                       & 20.3                       & 15.7                       & $\underset{(1)}{0.237}$          & $\underset{(1)}{0.221}$          & $\underset{(0)}{0.025}$          & $\underset{(0)}{0.100}$          & 2                         \\ \hline
\textbf{ML}   & Re-GHS  & 147.45 &	\textbf{4.004} &	70.98 &	\textbf{4.210}                & 9.7                        & 18.2                       & 10.5                       & 14.8                       & $\underset{(2)}{0.423}$          & $\underset{(2)}{0.459}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(2)}{0.375}$          & 6                         \\
              & Re-EGHS & 143.24 &	3.741 &	70.98 &	3.935                       & 7.0                        & 6.8                        & 10.5                       & 10.0                       & $\underset{(3)}{0.559}$          & $\underset{(3)}{0.637}$          & $\underset{(1)}{0.278}$          & $\underset{(2)}{0.367}$          & 9                         \\ \hline
\textbf{QLML} & Re-C1   & 148.54 &	3.935 &	74.22 &	4.172                        & 12.0                       & 20.7                       & 19.3                       & \textbf{21.3}              & $\underset{(3)}{0.533}$          & $\underset{(1)}{0.373}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.284}$          & 5                         \\
              & 2.5     & 149.57 &	3.818 &	73.78 &	3.975                       & 14.7                       & 15.8                       & 13.7                       & 12.0                       & $\underset{(2)}{0.483}$          & $\underset{(1)}{0.387}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.367}$          & 4                         \\
              & 5       & 147.64 &	3.810 &	74.37 &	3.989                        & 8.7                        & 15.3                       & 17.7                       & 17.7                       & $\underset{(2)}{0.489}$          & $\underset{(1)}{0.395}$          & $\underset{(1)}{0.219}$          & $\underset{(1)}{0.309}$          & 5                         \\
              & 10      & 148.48 &	3.885 &	72.11 &	4.090                        & 12.3                       & 18.8                       & 16.0                       & 19.0                       & $\underset{(2)}{0.458}$          & $\underset{(1)}{0.373}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.285}$          & 4                         \\
              & 15      & 149.65 &	3.965 &	74.60 &	4.195                        & 16.7                       & 19.5                       & 20.7                       & 21.0                       & $\underset{(2)}{0.467}$          & $\underset{(1)}{0.368}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.289}$          & 4                         \\
              & 20      & 149.17 &	3.965 &	74.95 &	4.207                       & 14.7                       & 20.8                       & 20.0                       & \textbf{21.3}              & $\underset{(2)}{0.454}$          & $\underset{(1)}{0.373}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(1)}{0.287}$          & 4                         \\ \hline
\textbf{QLML} & Re-EC1  & 145.64 &	3.768 &	68.12 &	3.900                        & 8.0                        & 6.0                        & {\color{blue}4.3} & 4.3                        & $\underset{(3)}{0.557}$          & $\underset{(2)}{0.565}$          & $\underset{(2)}{0.652}$          & $\underset{(2)}{0.674}$          & 9                         \\
              & 2.5     & 143.07 &	3.742 &	66.12 &	3.870                       & 4.7                        & 5.7                        & {\fbox{4.0}} & 4.2                        & $\underset{(3)}{0.563}$          & $\underset{(2)}{0.639}$          & $\underset{(3)}{0.593}$          & $\underset{(2)}{0.674}$          & 10                        \\
              & 5       & {\color{blue}141.82} & 3.734 &	65.73 &	3.868                       & {\fbox{3.0}} & {\color{blue}3.2} & {\fbox{4.0}} & 4.3                        & $\underset{(3)}{0.676}$          & $\underset{(3)}{0.661}$          & $\underset{(3)}{0.608}$          & $\underset{(3)}{0.571}$          & {\fbox{12}} \\
              & 10      & {\fbox{141.74}} & {\fbox{3.729}} & {\fbox{65.51}} & {\color{blue}3.860} & {\color{blue}4.0} & 3.5                        & 4.7                        & {\color{blue}4.0} & $\underset{(3)}{\fbox{0.791}}$   & $\underset{(3)}{\fbox{0.898}}$   & $\underset{(2)}{0.619}$          & $\underset{(3)}{\cb{0.706}}$     & {\color{blue}11} \\
              & 15      & 142.28                  & {\color{blue}3.730} & {\color{blue}65.71} & {\fbox{3.859}} & 5.0                        & {\fbox{1.7}} & 5.7                        & {\fbox{3.8}} & $\underset{(3)}{\cb{0.709}}$     & $\underset{(3)}{\cb{0.762}}$     & $\underset{(2)}{0.667}$          & $\underset{(3)}{\fbox{0.917}}$   & {\color{blue}11} \\
              & 20      & 143.21                 & 3.738 &	72.99 &	3.962                        & 7.7                        & 5.2                        & 13.3                       & 11.3                       & $\underset{(3)}{0.455}$          & $\underset{(2)}{0.619}$          & $\underset{(1)}{0.197}$          & $\underset{(2)}{0.421}$          & 8                         \\ \hline
\end{tabular}
}
\end{table}


==> all-assets.1day.tex <==

\begin{table}[htb]
\caption{\small 1-day risk forecasting results: average values across all assets. Key to table: \emph{Est.}: estimation method; \emph{Q$\alpha$}; average quantile loss value at the $\alpha\%$ ; \emph{J$\alpha$}; average joint loss value at the $\alpha\%$; \emph{R(L$\alpha$)}: average ranking of models under loss L at level $\alpha$; \emph{M(L$\alpha$)}: MCS p-value under loss L$\alpha$ (in brackets: number of times a model is included in the MCS); \emph{M(all)}: number of times a model is included in the MCS overall.\\}
\label{tab:allassets1day}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.65}
\small
%\begin{tabularx}{\textwidth}{*{15}{>{\centering\arraybackslash}X}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccc}
\hline
Est.          & Model   & Q2.5                           & J2.5                         & Q1                             & J1                           & R(Q2.5)                    & R(J2.5)                    & R(Q1)                      & R(J1)                      & M(Q2.5)                          & M(J2.5)                          & M(Q1)                            & M(J1)                            & M(all)                    \\ \hline
\textbf{ML}   & GHS     & 218.177                        & 2.777                        & 120.373                        & 3.139                        & 23.3                       & 19.8                       & 23.3                       & 16.7                       & $\underset{(0)}{\textbf{0.047}}$ & $\underset{(1)}{0.368}$          & $\underset{(1)}{0.292}$          & $\underset{(2)}{0.651}$          & \textbf{4}                \\
              & GJ-HS   & \textbf{220.958}               & \textbf{2.792}               & \textbf{121.910}               & 3.160                        & \textbf{26.3}              & \textbf{24.3}              & \textbf{26.0}              & \textbf{22.2}              & $\underset{(0)}{0.063}$          & $\underset{(1)}{0.342}$          & $\underset{(1)}{\textbf{0.263}}$ & $\underset{(2)}{0.622}$          & \textbf{4}                \\ \hline
\textbf{QL}   & IG1     & 215.038                        & 2.762                        & 117.550                        & 3.111                        & 16.3                       & 14.5                       & 18.3                       & 15.0                       & $\underset{(0)}{0.138}$          & $\underset{(1)}{0.413}$          & $\underset{(3)}{0.596}$          & $\underset{(3)}{0.684}$          & 7                         \\
              & 2.5      & 215.354                        & 2.767                        & 116.834                        & 3.104                        & 17.7                       & 17.5                       & 13.7                       & 13.3                       & $\underset{(1)}{0.211}$          & $\underset{(1)}{0.371}$          & $\underset{(3)}{0.589}$          & $\underset{(3)}{0.674}$          & 8                         \\
              & 5       & 217.493                        & 2.777                        & 117.578                        & 3.108                        & 23.0                       & 21.8                       & 16.7                       & 15.7                       & $\underset{(0)}{0.049}$          & $\underset{(1)}{0.355}$          & $\underset{(3)}{0.519}$          & $\underset{(3)}{0.650}$          & 7                         \\
              & 10      & 217.688                        & 2.778                        & 118.163                        & 3.136                        & 22.7                       & 22.3                       & 18.3                       & 19.0                       & $\underset{(0)}{0.054}$          & $\underset{(1)}{0.367}$          & $\underset{(3)}{0.461}$          & $\underset{(2)}{0.655}$          & 6                         \\
              & 15      & 217.127                        & 2.772                        & 118.608                        & 3.126                        & 20.3                       & 18.5                       & 21.0                       & 16.0                       & $\underset{(0)}{0.099}$          & $\underset{(2)}{0.478}$          & $\underset{(2)}{0.466}$          & $\underset{(3)}{0.737}$          & 7                         \\
              & 20      & 216.852                        & 2.769                        & 118.750                        & 3.114                        & 20.7                       & 19.0                       & 21.0                       & 17.0                       & $\underset{(0)}{0.085}$          & $\underset{(1)}{0.384}$          & $\underset{(3)}{0.437}$          & $\underset{(3)}{0.662}$          & 7                         \\
              & IGJR1   & 216.891                        & 2.775                        & 118.450                        & 3.137                        & 19.7                       & 19.3                       & 17.3                       & 19.3                       & $\underset{(1)}{0.231}$          & $\underset{(2)}{\textbf{0.246}}$ & $\underset{(3)}{0.579}$          & $\underset{(3)}{0.612}$          & 9                         \\
              & 2.5      & 216.188                        & 2.772                        & 118.309                        & 3.121                        & 19.0                       & 20.7                       & 19.0                       & 19.8                       & $\underset{(0)}{0.100}$          & $\underset{(1)}{0.367}$          & $\underset{(3)}{0.471}$          & $\underset{(3)}{0.631}$          & 7                         \\
              & 5       & 217.736                        & 2.774                        & 117.815                        & 3.115                        & 23.7                       & 20.3                       & 18.0                       & 16.3                       & $\underset{(0)}{0.067}$          & $\underset{(1)}{0.358}$          & $\underset{(3)}{0.489}$          & $\underset{(3)}{0.617}$          & 7                         \\
              & 10      & 216.100                        & 2.762                        & 116.789                        & 3.113                        & 19.7                       & 17.3                       & 13.3                       & 13.0                       & $\underset{(0)}{0.143}$          & $\underset{(2)}{0.535}$          & $\underset{(3)}{0.591}$          & $\underset{(3)}{0.765}$          & 8                         \\
              & 15      & 218.526                        & 2.779                        & 118.397                        & 3.131                        & 24.7                       & 22.5                       & 20.3                       & 18.8                       & $\underset{(0)}{0.065}$          & $\underset{(2)}{0.417}$          & $\underset{(2)}{0.464}$          & $\underset{(3)}{0.689}$          & 7                         \\
              & 20      & 217.446                        & 2.771                        & 118.761                        & 3.116                        & 24.0                       & 20.7                       & 21.3                       & 18.7                       & $\underset{(0)}{0.093}$          & $\underset{(1)}{0.381}$          & $\underset{(3)}{0.423}$          & $\underset{(3)}{0.620}$          & 7                         \\ \hline
\textbf{ML}   & Re-GHS  & 207.982                        & {\color{blue}2.712} & {\color{blue}114.128} & {\fbox{3.088}} & 6.3                        & 4.5                        & 8.3                        & {\fbox{7.8}} & $\underset{(3)}{\fbox{0.883}}$   & $\underset{(3)}{\cb{0.822}}$     & $\underset{(3)}{0.795}$          & $\underset{(3)}{0.933}$          & {\fbox{12}} \\
              & Re-EGHS & 208.113                        & 2.714                        & 114.516                        & 3.098                        & 5.5                        & {\color{blue}3.7} & 6.0                        & {\fbox{7.8}} & $\underset{(2)}{0.573}$          & $\underset{(3)}{0.799}$          & $\underset{(3)}{0.798}$          & $\underset{(3)}{\cb{0.935}}$     & {\color{blue}11} \\ \hline
\textbf{QLML} & Re-C1  & 208.443                        & 2.724                        & 116.604                        & 3.117                        & 8.2                        & 8.7                        & 13.3                       & 13.3                       & $\underset{(2)}{0.423}$          & $\underset{(2)}{0.670}$          & $\underset{(3)}{0.656}$          & $\underset{(3)}{0.789}$          & 10                        \\
              & 2.5      & 209.176                        & 2.737                        & 118.560                        & 3.153                        & 11.5                       & 16.2                       & 14.0                       & 13.8                       & $\underset{(1)}{0.249}$          & $\underset{(2)}{0.533}$          & $\underset{(2)}{0.559}$          & $\underset{(3)}{0.564}$          & 8                         \\
              & 5       & 208.573                        & 2.731                        & 116.644                        & 3.149                        & 9.2                        & 14.8                       & 13.7                       & 15.0                       & $\underset{(2)}{0.401}$          & $\underset{(3)}{0.699}$          & $\underset{(3)}{0.713}$          & $\underset{(3)}{0.619}$          & {\color{blue}11} \\
              & 10      & 208.819                        & 2.739                        & 121.520                        & 3.164                        & 9.8                        & 16.7                       & 16.3                       & 18.2                       & $\underset{(2)}{0.324}$          & $\underset{(2)}{0.477}$          & $\underset{(2)}{0.407}$          & $\underset{(2)}{\textbf{0.415}}$ & 8                         \\
              & 15      & 208.269                        & 2.749                        & 120.963                        & \textbf{3.199}               & 7.8                        & 14.7                       & 12.0                       & 12.7                       & $\underset{(2)}{0.456}$          & $\underset{(2)}{0.517}$          & $\underset{(2)}{0.675}$          & $\underset{(2)}{0.533}$          & 8                         \\
              & 20      & 209.734                        & 2.724                        & 117.214                        & 3.120                        & 10.7                       & 11.3                       & 9.7                        & 10.2                       & $\underset{(2)}{0.463}$          & $\underset{(3)}{0.763}$          & $\underset{(2)}{0.733}$          & $\underset{(3)}{0.892}$          & 10                        \\ \hline
\textbf{QLML} & Re-EC1  & {\color{blue}207.725} & 2.718                        & {\fbox{113.321}} & {\color{blue}3.095} & {\fbox{4.5}} & 6.0                        & {\color{blue}5.7} & 8.2                        & $\underset{(3)}{\cb{0.780}}$     & $\underset{(3)}{0.731}$          & $\underset{(3)}{\cb{0.863}}$     & $\underset{(3)}{0.791}$          & {\fbox{12}} \\
              & 2.5      & 208.363                        & 2.719                        & 114.443                        & 3.103                        & 6.2                        & 6.7                        & 7.0                        & 11.7                       & $\underset{(2)}{0.449}$          & $\underset{(2)}{0.692}$          & $\underset{(3)}{0.759}$          & $\underset{(3)}{0.806}$          & 10                        \\
              & 5       & 207.833                        & 2.719                        & 114.859                        & 3.101                        & 6.2                        & 5.5                        & 9.0                        & 12.2                       & $\underset{(2)}{0.542}$          & $\underset{(3)}{0.776}$          & $\underset{(3)}{0.759}$          & $\underset{(3)}{0.868}$          & {\color{blue}11} \\
              & 10      & 208.462                        & 2.722                        & 114.946                        & 3.110                        & 8.2                        & 8.5                        & 10.3                       & 13.3                       & $\underset{(2)}{0.459}$          & $\underset{(3)}{0.725}$          & $\underset{(3)}{0.727}$          & $\underset{(3)}{0.781}$          & {\color{blue}11} \\
              & 15      & 208.018                        & 2.721                        & 114.497                        & 3.117                        & 5.8                        & 7.8                        & 8.3                        & 13.0                       & $\underset{(2)}{0.490}$          & $\underset{(3)}{0.752}$          & $\underset{(3)}{0.852}$          & $\underset{(3)}{0.755}$          & {\color{blue}11} \\
              & 20      & {\fbox{207.715}} & {\fbox{2.711}} & 114.236                        & {\fbox{3.088}} & {\color{blue}5.2} & {\fbox{2.3}} & {\fbox{4.7}} & {\color{blue}8.0} & $\underset{(2)}{0.605}$          & $\underset{(3)}{\fbox{0.957}}$   & $\underset{(3)}{\fbox{0.865}}$   & $\underset{(3)}{\fbox{0.997}}$   & {\color{blue}11} \\ \hline
\end{tabular}
}
\end{table}


==> all-markets.10days.tex <==
\begin{table}[htb]
\caption{\small 10-day risk forecasting results: average values across all markets. Key to table: \emph{Est.}: estimation method; \emph{Q$\alpha$}; average quantile loss value at the $\alpha\%$ ; \emph{J$\alpha$}; average joint loss value at the $\alpha\%$; \emph{R(L$\alpha$)}: average ranking of models under loss L at level $\alpha$; \emph{M(L$\alpha$)}: MCS p-value under loss L$\alpha$ (in brackets: number of times a model is included in the MCS); \emph{M(all)}: number of times a model is included in the MCS overall.\\}
\label{tab:allmarkets10day}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.65}
\small
%\begin{tabularx}{\textwidth}{*{15}{>{\centering\arraybackslash}X}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccc}
\hline
Est.          & Model   & Q2.5                          & J2.5                         & Q1                            & J1                           & R(Q2.5)                    & R(J2.5)                    & R(Q1)                      & R(J1)                      & M(Q2.5)                          & M(J2.5)                          & M(Q1)                            & M(J1)                           & M(all)                    \\ \hline
\textbf{ML}   & GHS     & 95.362                        & 3.360                        & 49.119                        & 3.620                        & 19.0                       & 24.5                       & 13.7                       & 20.0                       & $\underset{(3)}{0.515}$          & $\underset{(3)}{0.397}$          & $\underset{(2)}{0.414}$          & $\underset{(3)}{0.513}$         & {\fbox{11}} \\
              & GJ-HS   & {\color{blue}91.101} & {\fbox{3.252}} & 46.871                        & 3.493                        & {\fbox{4.3}} & {\fbox{4.7}} & {\color{blue}4.3} & 6.8                        & $\underset{(3)}{\fbox{0.860}}$   & $\underset{(3)}{\cb{0.811}}$     & $\underset{(2)}{\cb{0.597}}$     & $\underset{(3)}{0.699}$         & {\fbox{11}} \\ \hline
\textbf{QL}   & IG1     & 93.672                        & 3.285                        & {\color{blue}46.869} & 3.501                        & 13.0                       & 10.3                       & 7.0                        & 7.3                        & $\underset{(3)}{0.631}$          & $\underset{(3)}{0.496}$          & $\underset{(2)}{\fbox{0.660}}$   & $\underset{(3)}{0.747}$         & {\fbox{11}} \\
              & 2.5     & 93.574                        & 3.286                        & 48.042                        & 3.529                        & 13.7                       & 10.2                       & 9.7                        & 10.7                       & $\underset{(3)}{0.616}$          & $\underset{(3)}{0.496}$          & $\underset{(2)}{0.424}$          & $\underset{(3)}{0.687}$         & {\fbox{11}} \\
              & 5       & 93.488                        & 3.295                        & 48.405                        & 3.560                        & 11.7                       & 14.3                       & 12.7                       & 15.3                       & $\underset{(3)}{0.568}$          & $\underset{(3)}{0.477}$          & $\underset{(1)}{0.35}$           & $\underset{(3)}{0.6}$           & {\color{blue}10} \\
              & 10      & 92.873                        & 3.308                        & 48.609                        & 3.591                        & 13.7                       & 17.0                       & 12.7                       & 19.0                       & $\underset{(3)}{0.595}$          & $\underset{(3)}{0.485}$          & $\underset{(1)}{0.347}$          & $\underset{(3)}{0.545}$         & {\color{blue}10} \\
              & 15      & 92.056                        & 3.319                        & 49.964                        & 3.642                        & 12.3                       & 19.5                       & 14.7                       & 21.3                       & $\underset{(3)}{0.689}$          & $\underset{(3)}{0.479}$          & $\underset{(1)}{0.319}$          & $\underset{(3)}{0.5}$           & {\color{blue}10} \\
              & 20      & 93.516                        & 3.331                        & 49.924                        & 3.640                        & 16.3                       & 21.0                       & 14.7                       & 24.0                       & $\underset{(3)}{0.525}$          & $\underset{(3)}{0.452}$          & $\underset{(1)}{0.341}$          & $\underset{(3)}{0.518}$         & {\color{blue}10} \\
              & IGJR1   & 94.761                        & 3.279                        & 47.447                        & {\color{blue}3.485} & 18.7                       & 11.2                       & 11.0                       & {\color{blue}6.3} & $\underset{(3)}{0.6}$            & $\underset{(3)}{0.493}$          & $\underset{(2)}{0.544}$          & $\underset{(3)}{\cb{0.763}}$    & {\fbox{11}} \\
              & 2.5     & 92.822                        & 3.263                        & {\fbox{46.792}} & {\fbox{3.470}} & 14.7                       & 7.0                        & {\fbox{3.7}} & {\fbox{3.8}} & $\underset{(3)}{0.611}$          & $\underset{(3)}{0.693}$          & $\underset{(2)}{0.577}$          & $\underset{(3)}{\fbox{0.769}}$  & {\fbox{11}} \\
              & 5       & 92.261                        & 3.265                        & 47.860                        & 3.508                        & 11.7                       & 8.7                        & 10.7                       & 9.3                        & $\underset{(3)}{0.623}$          & $\underset{(3)}{0.489}$          & $\underset{(1)}{0.311}$          & $\underset{(3)}{0.626}$         & {\color{blue}10} \\
              & 10      & {\fbox{90.952}} & {\color{blue}3.258} & 47.707                        & 3.526                        & {\color{blue}5.7} & {\color{blue}5.5} & 10.0                       & 11.0                       & $\underset{(3)}{\cb{0.819}}$     & $\underset{(3)}{\fbox{0.819}}$   & $\underset{(2)}{0.583}$          & $\underset{(3)}{0.625}$         & {\fbox{11}} \\
              & 15      & 91.844                        & 3.289                        & 49.085                        & 3.580                        & 7.3                        & 11.0                       & 12.7                       & 11.3                       & $\underset{(3)}{0.765}$          & $\underset{(3)}{0.661}$          & $\underset{(2)}{0.519}$          & $\underset{(3)}{0.69}$          & {\fbox{11}} \\
              & 20      & 91.464                        & 3.273                        & 49.523                        & 3.562                        & 8.0                        & 9.3                        & 11.7                       & 12.3                       & $\underset{(3)}{0.767}$          & $\underset{(3)}{0.48}$           & $\underset{(1)}{0.29}$           & $\underset{(3)}{0.577}$         & {\color{blue}10} \\ \hline
\textbf{ML}   & Re-GHS  & 96.274                        & 3.357                        & 51.558                        & 3.681                        & 19.7                       & 20.5                       & 19.5                       & 18.7                       & $\underset{(3)}{0.529}$          & $\underset{(3)}{0.359}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(3)}{0.493}$         & 9                         \\
              & Re-EGHS & 94.847                        & 3.285                        & 51.558                        & 3.586                        & 11.3                       & 11.5                       & 19.5                       & 16.3                       & $\underset{(2)}{0.634}$          & $\underset{(3)}{0.644}$          & $\underset{(2)}{0.339}$          & $\underset{(3)}{0.426}$         & {\color{blue}10} \\ \hline
\textbf{QLML} & Re-C1   & 96.297                        & 3.338                        & 51.753                        & 3.650                        & 19.3                       & 18.0                       & 20.3                       & 17.3                       & $\underset{(3)}{0.48}$           & $\underset{(3)}{0.453}$          & $\underset{(0)}{0.057}$          & $\underset{(2)}{\textbf{0.395}}$ & \textbf{8}                \\
              & 2.5     & 96.999                        & 3.372                        & 52.644                        & 3.716                        & 22.0                       & 23.3                       & \textbf{26.0}              & 23.0                       & $\underset{(2)}{0.413}$          & $\underset{(3)}{0.376}$          & $\underset{(1)}{0.107}$          & $\underset{(3)}{0.583}$         & 9                         \\
              & 5       & 96.669                        & 3.367                        & 52.268                        & 3.711                        & 19.7                       & 21.7                       & 22.0                       & 22.3                       & $\underset{(3)}{0.425}$          & $\underset{(3)}{0.372}$          & $\underset{(1)}{0.133}$          & $\underset{(3)}{0.469}$         & {\color{blue}10} \\
              & 10      & 96.095                        & 3.362                        & 51.499                        & 3.698                        & 19.0                       & 21.7                       & 20.3                       & 21.0                       & $\underset{(3)}{0.513}$          & $\underset{(3)}{0.327}$          & $\underset{(1)}{0.167}$          & $\underset{(3)}{0.501}$         & {\color{blue}10} \\
              & 15      & 96.936                        & 3.374                        & 52.608                        & 3.723                        & 22.3                       & 23.5                       & 25.3                       & 24.0                       & $\underset{(3)}{0.371}$          & $\underset{(3)}{0.303}$          & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(3)}{0.419}$         & 9                         \\
              & 20      & \textbf{97.489}               & \textbf{3.383}               & \textbf{53.211}               & \textbf{3.736}               & \textbf{24.7}              & \textbf{26.2}              & 25.7                       & \textbf{24.3}              & $\underset{(2)}{\textbf{0.299}}$ & $\underset{(3)}{\textbf{0.291}}$ & $\underset{(0)}{\textbf{0.000}}$ & $\underset{(3)}{0.412}$         & \textbf{8}                \\ \hline
\textbf{QLML} & Re-EC1  & 95.370                        & 3.280                        & 48.897                        & 3.498                        & 16.3                       & 10.0                       & 11.0                       & 7.3                        & $\underset{(3)}{0.553}$          & $\underset{(3)}{0.485}$          & $\underset{(1)}{0.366}$          & $\underset{(3)}{0.663}$         & {\color{blue}10} \\
              & 2.5     & 94.871                        & 3.278                        & 49.205                        & 3.514                        & 13.0                       & 9.7                        & 12.3                       & 8.7                        & $\underset{(2)}{0.595}$          & $\underset{(3)}{0.479}$          & $\underset{(1)}{0.29}$           & $\underset{(3)}{0.663}$         & 9                         \\
              & 5       & 95.090                        & 3.284                        & 49.580                        & 3.525                        & 14.7                       & 12.8                       & 13.3                       & 10.7                       & $\underset{(2)}{0.611}$          & $\underset{(3)}{0.451}$          & $\underset{(1)}{0.243}$          & $\underset{(3)}{0.585}$         & 9                         \\
              & 10      & 94.365                        & 3.273                        & 49.068                        & 3.515                        & 9.3                        & 9.3                        & 13.0                       & 10.3                       & $\underset{(3)}{0.664}$          & $\underset{(3)}{0.485}$          & $\underset{(1)}{0.233}$          & $\underset{(3)}{0.636}$         & {\color{blue}10} \\
              & 15      & 94.943                        & 3.283                        & 49.561                        & 3.529                        & 11.0                       & 10.8                       & 12.7                       & 11.0                       & $\underset{(2)}{0.629}$          & $\underset{(3)}{0.433}$          & $\underset{(1)}{0.25}$           & $\underset{(3)}{0.629}$         & 9                         \\
              & 20      & 95.230                        & 3.285                        & 50.043                        & 3.534                        & 13.7                       & 12.8                       & 16.0                       & 12.3                       & $\underset{(2)}{0.627}$          & $\underset{(3)}{0.473}$          & $\underset{(1)}{0.213}$          & $\underset{(3)}{0.608}$         & 9                         \\ \hline
\end{tabular}
}
\end{table}

==> all-markets.1day.tex <==

\begin{table}[htb]
\caption{\small 1-day risk forecasting results: average values across all markets. Key to table: \emph{Est.}: estimation method; \emph{Q$\alpha$}; average quantile loss value at the $\alpha\%$ ; \emph{J$\alpha$}; average joint loss value at the $\alpha\%$; \emph{R(L$\alpha$)}: average ranking of models under loss L at level $\alpha$; \emph{M(L$\alpha$)}: MCS p-value under loss L$\alpha$ (in brackets: number of times a model is included in the MCS); \emph{M(all)}: number of times a model is included in the MCS overall. \\}
\label{tab:allmarkets1day}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.65}
\small
%\begin{tabularx}{\textwidth}{*{15}{>{\centering\arraybackslash}X}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccccc}
\hline
Est.  & Model   & Q2.5                           & J2.5                         & Q1                            & J1                           & R(Q2.5)                    & R(J2.5)                    & R(Q1)                      & R(J1)                      & M(Q2.5)                          & M(J2.5)                         & M(Q1)                            & M(J1)                            & M(all)                    \\ \hline
\textbf{ML}      & GHS     & 113.347                        & 2.062                        & 56.124                        & 2.275                        & 15.7                       & 19.2                       & 15.3                       & 19.0                       & $\underset{(2)}{0.362}$          & $\underset{(1)}{0.246}$         & $\underset{(2)}{0.445}$          & $\underset{(2)}{0.410}$          & 7                         \\
      & GJ-HS   & 110.235                        & 2.032                        & 54.966                        & 2.267                        & 6.7                        & 10.8                       & 11.7                       & 17.3                       & $\underset{(3)}{0.816}$          & $\underset{(1)}{0.472}$         & $\underset{(3)}{0.818}$          & $\underset{(2)}{0.505}$          & 9                         \\ \hline
\textbf{QL}      & IG1     & 112.482                        & 2.051                        & 55.088                        & 2.254                        & 14.7                       & 16.3                       & 11.3                       & 16.8                       & $\underset{(2)}{0.499}$          & $\underset{(1)}{0.397}$         & $\underset{(2)}{0.687}$          & $\underset{(2)}{0.615}$          & 7                         \\
      & 2.5     & 113.094                        & 2.056                        & 55.497                        & 2.254                        & 17.0                       & 18.7                       & 14.0                       & 17.3                       & $\underset{(2)}{0.447}$          & $\underset{(1)}{0.387}$         & $\underset{(2)}{0.682}$          & $\underset{(2)}{0.578}$          & 7                         \\
      & 5       & 113.406                        & 2.064                        & 56.490                        & 2.275                        & 17.3                       & 20.3                       & 17.3                       & 19.7                       & $\underset{(2)}{0.353}$          & $\underset{(1)}{0.285}$         & $\underset{(2)}{0.413}$          & $\underset{(2)}{0.497}$          & 7                         \\
      & 10      & 114.234                        & 2.067                        & 56.660                        & 2.287                        & 18.0                       & 19.7                       & 14.3                       & 18.2                       & $\underset{(2)}{0.290}$          & $\underset{(1)}{0.170}$         & $\underset{(1)}{0.375}$          & $\underset{(1)}{0.319}$          & 5                         \\
      & 15      & 116.347                        & 2.085                        & 58.621                        & 2.314                        & 26.3                       & 22.3                       & \textbf{25.3}              & 21.3                       & $\underset{(1)}{\textbf{0.214}}$ & $\underset{(1)}{\textbf{0.134}}$ & $\underset{(1)}{\textbf{0.244}}$ & $\underset{(1)}{0.247}$          & \textbf{4}                \\
      & 20      & \textbf{116.852}               & \textbf{2.091}               & \textbf{59.436}               & \textbf{2.329}               & \textbf{26.7}              & \textbf{24.2}              & \textbf{25.3}              & \textbf{24.3}              & $\underset{(2)}{0.246}$          & $\underset{(1)}{0.138}$         & $\underset{(2)}{0.327}$          & $\underset{(1)}{\textbf{0.215}}$ & 6                         \\
      & IGJR1   & 113.538                        & 2.062                        & 55.914                        & 2.275                        & 18.7                       & 19.8                       & 15.0                       & 19.7                       & $\underset{(2)}{0.419}$          & $\underset{(1)}{0.371}$         & $\underset{(2)}{0.592}$          & $\underset{(2)}{0.561}$          & 7                         \\
      & 2.5     & 112.787                        & 2.068                        & 56.374                        & 2.291                        & 15.3                       & 19.5                       & 17.0                       & 19.0                       & $\underset{(2)}{0.509}$          & $\underset{(1)}{0.355}$         & $\underset{(2)}{0.531}$          & $\underset{(2)}{0.443}$          & 7                         \\
      & 5       & 112.163                        & 2.054                        & 56.680                        & 2.295                        & 13.2                       & 16.5                       & 19.3                       & 19.7                       & $\underset{(3)}{0.519}$          & $\underset{(1)}{0.374}$         & $\underset{(2)}{0.453}$          & $\underset{(1)}{0.441}$          & 7                         \\
      & 10      & 111.104                        & 2.043                        & 55.279                        & 2.274                        & 10.3                       & 16.8                       & 13.3                       & 17.3                       & $\underset{(3)}{0.717}$          & $\underset{(1)}{0.409}$         & $\underset{(3)}{0.710}$          & $\underset{(2)}{0.423}$          & 9                         \\
      & 15      & 113.864                        & 2.065                        & 56.870                        & 2.307                        & 19.7                       & 17.3                       & 18.0                       & 17.7                       & $\underset{(3)}{0.516}$          & $\underset{(2)}{0.326}$         & $\underset{(2)}{0.501}$          & $\underset{(2)}{0.369}$          & 9                         \\
      & 20      & 115.052                        & 2.074                        & 57.711                        & 2.315                        & 23.3                       & 20.3                       & 21.0                       & 20.8                       & $\underset{(2)}{0.318}$          & $\underset{(1)}{0.213}$         & $\underset{(3)}{0.510}$          & $\underset{(1)}{0.263}$          & 7                         \\ \hline
 \textbf{ML}     & Re-GHS  & 113.881                        & 2.045                        & 57.167                        & 2.276                        & 18.2                       & 16.3                       & 17.7                       & 15.3                       & $\underset{(2)}{0.405}$          & $\underset{(2)}{0.299}$         & $\underset{(3)}{0.461}$          & $\underset{(2)}{0.411}$          & 9                         \\
      & Re-EGHS & 109.969                        & 1.997                        & 54.444                        & 2.204                        & 7.0                        & 6.3                        & 9.3                        & 7.8                        & $\underset{(3)}{0.797}$          & $\underset{(3)}{0.683}$         & $\underset{(3)}{0.821}$          & $\underset{(3)}{0.798}$          & {\fbox{12}} \\ \hline
\textbf{QLML}      & Re-C1   & 114.135                        & 2.046                        & 57.203                        & 2.273                        & 19.7                       & 17.5                       & 18.3                       & 14.3                       & $\underset{(2)}{0.353}$          & $\underset{(2)}{0.257}$         & $\underset{(3)}{0.427}$          & $\underset{(1)}{0.386}$          & 8                         \\
      & 2.5     & 114.299                        & 2.047                        & 57.383                        & 2.273                        & 19.0                       & 14.8                       & 20.0                       & 13.8                       & $\underset{(3)}{0.503}$          & $\underset{(1)}{0.323}$         & $\underset{(3)}{0.591}$          & $\underset{(3)}{0.502}$          & {\color{blue}10} \\
      & 5       & 113.672                        & 2.044                        & 56.811                        & 2.274                        & 17.3                       & 15.3                       & 16.3                       & 14.0                       & $\underset{(2)}{0.457}$          & $\underset{(2)}{0.429}$         & $\underset{(3)}{0.591}$          & $\underset{(2)}{0.533}$          & 9                         \\
      & 10      & 113.929                        & 2.044                        & 57.280                        & 2.275                        & 18.3                       & 15.5                       & 19.0                       & 14.2                       & $\underset{(3)}{0.408}$          & $\underset{(2)}{0.282}$         & $\underset{(3)}{0.459}$          & $\underset{(1)}{0.385}$          & 9                         \\
      & 15      & 114.370                        & 2.047                        & 57.381                        & 2.277                        & 21.7                       & 18.3                       & 20.7                       & 14.8                       & $\underset{(2)}{0.391}$          & $\underset{(2)}{0.281}$         & $\underset{(3)}{0.479}$          & $\underset{(1)}{0.390}$          & 8                         \\
      & 20      & 113.946                        & 2.043                        & 57.132                        & 2.271                        & 18.3                       & 16.0                       & 19.3                       & 13.3                       & $\underset{(3)}{0.465}$          & $\underset{(2)}{0.317}$         & $\underset{(3)}{0.529}$          & $\underset{(1)}{0.440}$          & 9                         \\ \hline
\textbf{QLML} & Re-EC1  & 109.824                        & 1.996                        & 54.306                        & 2.205                        & 6.0                        & 5.2                        & 8.0                        & 8.7                        & $\underset{(3)}{0.801}$          & $\underset{(3)}{0.683}$         & $\underset{(3)}{0.885}$          & $\underset{(3)}{0.816}$          & {\fbox{12}} \\
      & 2.5     & 109.417                        & 1.996                        & 53.630                        & 2.201                        & {\fbox{3.0}} & 4.2                        & 6.0                        & 7.8                        & $\underset{(3)}{0.795}$          & $\underset{(3)}{0.686}$         & $\underset{(3)}{0.951}$          & $\underset{(3)}{0.901}$          & {\fbox{12}} \\
      & 5       & 109.092                        & 1.993                        & 53.567                        & 2.199                        & 4.0                        & 4.2                        & 5.3                        & 6.7                        & $\underset{(3)}{0.831}$          & $\underset{(3)}{0.683}$         & $\underset{(3)}{0.922}$          & $\underset{(3)}{0.839}$          & {\fbox{12}} \\
      & 10      & {\fbox{108.967}} & {\fbox{1.989}} & {\color{blue}53.306} & {\color{blue}2.187} & 4.0                        & {\fbox{3.2}} & {\color{blue}2.3} & {\color{blue}2.0} & $\underset{(3)}{\fbox{0.951}}$   & $\underset{(3)}{\fbox{0.885}}$  & $\underset{(3)}{\cb{0.960}}$     & $\underset{(3)}{\fbox{0.975}}$   & {\fbox{12}} \\
      & 15      & {\color{blue}109.008} & {\color{blue}1.992} & 53.396                        & 2.194                        & {\color{blue}3.3} & {\color{blue}3.5} & 3.3                        & 3.7                        & $\underset{(3)}{\cb{0.869}}$     & $\underset{(3)}{\cb{0.793}}$    & $\underset{(3)}{\cb{0.960}}$     & $\underset{(3)}{0.904}$          & {\fbox{12}} \\
      & 20      & 109.056                        & {\color{blue}1.992} & {\fbox{53.249}} & {\fbox{2.186}} & {\color{blue}3.3} & 3.8                        & {\fbox{2.0}} & {\fbox{1.3}} & $\underset{(3)}{0.832}$          & $\underset{(3)}{0.683}$         & $\underset{(3)}{\fbox{0.991}}$   & $\underset{(3)}{\cb{0.974}}$     & {\fbox{12}} \\ \hline
\end{tabular}
}
\end{table}

